The local ultraviolet signature of Type Ia supernova environments from HST and MUSE

The local environment of a Type Ia supernova (SN~Ia) traces the local stellar-population age (a statistical proxy for the progenitor age), star formation, dust, and chemical enrichment that may influence both its light-curve properties and its standardized luminosity. We assemble a homogeneous explosion-site dataset to test how near-ultraviolet (UV) imaging combined with optical integral-field spectroscopy improves the characterization of SN~Ia environments and their connection to SN~Ia observables. We analyze 340 low-redshift SN~Ia explosion sites observed with HST/WFC3 in F275W together with matched VLT/MUSE spectroscopy. For each site we measure local photometry and extract a 1~kpc-aperture spectrum, model the stellar continuum with STARLIGHT in a joint UV+optical fit, derive local stellar and gas-phase properties, and fit the SN light curves with sncosmo/SALT3-NIR. UV emission is detected at 235 of the 337 sites with valid HST imaging. The UV- and H$\alpha$-based star-formation-rate surface densities are strongly correlated, with the UV estimates systematically higher by about 0.5 dex. Including the UV constraint in the STARLIGHT fit shifts local luminosity-weighted ages toward older values by a median of $+0.20$ dex for UV detections and $+0.45$ dex for UV non-detections, showing that UV data help break age--dust--metallicity degeneracies and substantially alter and tighten the inferred local stellar-population ages within the adopted modelling framework. Consistently, F275W$-r$ is very strongly correlated with the joint-fit stellar age. Within the 169-SN~Ia calibration sample, the joint stellar age, the H$\alpha$ specific star-formation rate (sSFR), and the UV sSFR all correlate strongly with the SALT3 stretch parameter $x_1$, with significances above $6.8\sigma$. (abridged)

==> bibtex/table_env_sncosmo_median_split_summary_sideways_calibration_only.tex <==
% Merged median-split + correlations + robustness (landscape). Requires \usepackage{rotating}.
\begin{sidewaystable*}
\centering
\caption{Median-split and linear-relation diagnostics for $x_1$, $c$ and HR$_{\rm SALT}$ versus the twelve local tracers (169-object Tripp-calibration sample). The left block (``Two-bin'') characterizes the median split: $N$, the split value (``x cut''), the low/high-bin medians with robust errors, their difference and its significance $\sigma$, and two robustness checks of that significance: its range under a 30th--70th-percentile ``threshold'' scan and the ``censored''-MC value obtained when the UV non-detections are resampled beyond their limits (UV-based tracers only), quoted as the most conservative (lowest) value across the three draw prescriptions of Sect.~\ref{sec:lcenv}. The right block (``Linear-relation'') treats both variables as continuous over the $N_{\rm det}$ detections: the Pearson $r$, Spearman $\rho$ and Kendall $\tau$ coefficients (two-sided $p$ in parentheses) and a maximum-likelihood linear fit (errors in both variables plus an intrinsic-scatter term), the slope $b\pm\sigma_b$ (per dex, or per mag for F275W$-r$), its significance ``regression''$\,=|b/\sigma_b|$, and the intrinsic scatter $\sigma_{\rm int}$. Limits enter the median split at their limit values but not the correlations ($N_{\rm det}\le N$). All methods are defined in Sect.~\ref{sec:lcenv}.}
\label{tab:env_sncosmo_median_split_summary_calibration}
\label{tab:major2_rank}
\label{tab:major2_robust}
\label{tab:regression_slopes}
\scriptsize
\setlength{\tabcolsep}{3pt}
\resizebox{\textheight}{!}{
\begin{tabular}{ll|rrlllrcc|rlllrcc}
\hline\hline
\multicolumn{2}{c|}{} & \multicolumn{8}{c|}{Two-bin (median-split) statistics} & \multicolumn{7}{c}{Linear-relation statistics} \\
\cline{3-10}\cline{11-17}
y variable & x variable & N & x cut & low bin & high bin & Difference (h-l) & $\sigma$ & threshold & censored & $N_{\rm det}$ & Pearson $r$\,($p$) & Spearman $\rho$\,($p$) & Kendall $\tau$\,($p$) & $b\pm\sigma_b$ & regression & $\sigma_{\rm int}$ \\
 & & & & & & & & scan ($\sigma$) & MC ($\sigma$) & & & & & & ($\sigma$) & \\
\hline
x1 & 12+$\log$ (O/H) & 163 & 8.684 & $0.232\pm0.135$ & $-0.437\pm0.159$ & $-0.669\pm0.209$ & $3.21$ & $1.93$--$6.67$ & \ldots  & 163 & $-0.239$\,($2{\times}10^{-3}$) & $-0.257$\,($9{\times}10^{-4}$) & $-0.171$\,($1{\times}10^{-3}$) & $-1.44\pm0.54$ & $2.68$ & 1.153 \\
 & F275W-$r$ & 166 & 2.151 & $0.601\pm0.103$ & $-0.507\pm0.138$ & $-1.108\pm0.172$ & $6.44$ & $5.24$--$6.77$ & $4.01$  & 117 & $-0.418$\,($3{\times}10^{-6}$) & $-0.411$\,($4{\times}10^{-6}$) & $-0.295$\,($2{\times}10^{-6}$) & $-0.305\pm0.077$ & $3.95$ & 1.020 \\
 & $\log \Sigma$SFR$_{H\alpha}$ & 163 & -3.145 & $-0.382\pm0.191$ & $0.126\pm0.112$ & $0.509\pm0.222$ & $2.29$ & $0.12$--$2.90$ & \ldots  & 163 & $+0.107$\,($0.17$) & $+0.096$\,($0.22$) & $+0.060$\,($0.25$) & $0.119\pm0.086$ & $1.38$ & 1.189 \\
 & $\log \Sigma$SFR$_{UV}$ & 169 & -2.49 & $-0.306\pm0.161$ & $0.309\pm0.127$ & $0.615\pm0.205$ & $3.00$ & $1.83$--$3.32$ & $2.35$  & 119 & $+0.251$\,($6{\times}10^{-3}$) & $+0.268$\,($3{\times}10^{-3}$) & $+0.179$\,($4{\times}10^{-3}$) & $0.51\pm0.18$ & $2.86$ & 1.091 \\
 & $\log$ EW$_{H_\alpha}$ & 162 & 0.9167 & $-0.539\pm0.190$ & $0.380\pm0.102$ & $0.920\pm0.215$ & $4.27$ & $3.52$--$7.36$ & \ldots  & 162 & $+0.397$\,($2{\times}10^{-7}$) & $+0.392$\,($2{\times}10^{-7}$) & $+0.270$\,($4{\times}10^{-7}$) & $0.61\pm0.12$ & $5.18$ & 1.084 \\
 & $\log M$ & 169 & 7.907 & $0.551\pm0.130$ & $-0.395\pm0.146$ & $-0.946\pm0.196$ & $4.84$ & $4.27$--$5.68$ & \ldots  & 169 & $-0.361$\,($1{\times}10^{-6}$) & $-0.358$\,($2{\times}10^{-6}$) & $-0.246$\,($2{\times}10^{-6}$) & $-0.448\pm0.100$ & $4.50$ & 1.106 \\
 & $Z_L$ & 169 & 0.02498 & $0.325\pm0.137$ & $-0.262\pm0.144$ & $-0.587\pm0.199$ & $2.95$ & $1.65$--$3.63$ & \ldots  & 169 & $-0.112$\,($0.15$) & $-0.136$\,($0.077$) & $-0.095$\,($0.068$) & $-9.7\pm6.4$ & $1.52$ & 1.179 \\
 & $Z_M$ & 169 & 0.02318 & $0.079\pm0.150$ & $-0.025\pm0.129$ & $-0.104\pm0.198$ & $0.52$ & $0.05$--$2.39$ & \ldots  & 169 & $-0.027$\,($0.73$) & $-0.037$\,($0.64$) & $-0.031$\,($0.56$) & $-2.2\pm6.3$ & $0.34$ & 1.187 \\
 & $\log$ sSFR$_{H\alpha}$ & 163 & -10.38 & $-0.817\pm0.162$ & $0.546\pm0.106$ & $1.363\pm0.194$ & $7.04$ & $4.27$--$8.39$ & \ldots  & 163 & $+0.452$\,($1{\times}10^{-9}$) & $+0.461$\,($6{\times}10^{-10}$) & $+0.321$\,($1{\times}10^{-9}$) & $0.54\pm0.11$ & $5.09$ & 1.063 \\
 & $\log$ sSFR$_{UV}$ & 169 & -9.713 & $-0.638\pm0.155$ & $0.612\pm0.097$ & $1.250\pm0.183$ & $6.84$ & $5.55$--$7.41$ & $4.78$  & 119 & $+0.506$\,($5{\times}10^{-9}$) & $+0.496$\,($1{\times}10^{-8}$) & $+0.347$\,($2{\times}10^{-8}$) & $0.63\pm0.11$ & $5.72$ & 0.962 \\
 & $\log t_L$ & 169 & 8.807 & $0.606\pm0.098$ & $-0.762\pm0.149$ & $-1.368\pm0.179$ & $7.66$ & $5.39$--$8.18$ & \ldots  & 169 & $-0.475$\,(${<}10^{-10}$) & $-0.486$\,(${<}10^{-10}$) & $-0.344$\,(${<}10^{-10}$) & $-0.80\pm0.13$ & $6.27$ & 1.038 \\
 & $\log t_M$ & 169 & 9.227 & $0.401\pm0.118$ & $-0.507\pm0.164$ & $-0.909\pm0.202$ & $4.50$ & $2.81$--$6.20$ & \ldots  & 169 & $-0.380$\,($4{\times}10^{-7}$) & $-0.358$\,($2{\times}10^{-6}$) & $-0.248$\,($2{\times}10^{-6}$) & $-0.60\pm0.10$ & $5.85$ & 1.087 \\
\hline
c & 12+$\log$ (O/H) & 163 & 8.684 & $0.003\pm0.008$ & $0.021\pm0.010$ & $0.018\pm0.012$ & $1.45$ & $0.82$--$3.27$ & \ldots  & 163 & $+0.202$\,($1{\times}10^{-2}$) & $+0.217$\,($5{\times}10^{-3}$) & $+0.149$\,($5{\times}10^{-3}$) & $0.092\pm0.035$ & $2.65$ & 0.087 \\
 & F275W-$r$ & 166 & 2.151 & $-0.003\pm0.009$ & $0.025\pm0.008$ & $0.028\pm0.012$ & $2.35$ & $1.62$--$2.89$ & $0.51$  & 117 & $+0.093$\,($0.32$) & $+0.135$\,($0.15$) & $+0.089$\,($0.15$) & $0.0052\pm0.0050$ & $1.04$ & 0.088 \\
 & $\log \Sigma$SFR$_{H\alpha}$ & 163 & -3.145 & $0.007\pm0.007$ & $0.013\pm0.010$ & $0.007\pm0.012$ & $0.53$ & $0.08$--$2.42$ & \ldots  & 163 & $+0.178$\,($0.023$) & $+0.157$\,($0.045$) & $+0.105$\,($0.046$) & $0.0148\pm0.0067$ & $2.22$ & 0.088 \\
 & $\log \Sigma$SFR$_{UV}$ & 169 & -2.49 & $0.019\pm0.007$ & $-0.003\pm0.009$ & $-0.022\pm0.011$ & $1.95$ & $0.30$--$1.95$ & $0.81$  & 119 & $+0.062$\,($0.5$) & $+0.057$\,($0.54$) & $+0.025$\,($0.68$) & $0.010\pm0.016$ & $0.63$ & 0.089 \\
 & $\log$ EW$_{H_\alpha}$ & 162 & 0.9167 & $0.017\pm0.008$ & $0.003\pm0.010$ & $-0.014\pm0.013$ & $1.10$ & $0.05$--$1.10$ & \ldots  & 162 & $-4{\times}10^{-4}$\,($1$) & $-0.011$\,($0.89$) & $-0.015$\,($0.77$) & $-0.000\pm0.010$ & $0.00$ & 0.089 \\
 & $\log M$ & 169 & 7.907 & $-0.009\pm0.009$ & $0.031\pm0.009$ & $0.040\pm0.012$ & $3.29$ & $2.40$--$3.87$ & \ldots  & 169 & $+0.273$\,($3{\times}10^{-4}$) & $+0.321$\,($2{\times}10^{-5}$) & $+0.225$\,($1{\times}10^{-5}$) & $0.0253\pm0.0068$ & $3.73$ & 0.085 \\
 & $Z_L$ & 169 & 0.02498 & $0.011\pm0.009$ & $0.003\pm0.008$ & $-0.008\pm0.012$ & $0.66$ & $0.02$--$0.66$ & \ldots  & 169 & $-0.008$\,($0.92$) & $7{\times}10^{-6}$\,($1$) & $+0.003$\,($0.96$) & $-0.05\pm0.54$ & $0.10$ & 0.089 \\
 & $Z_M$ & 169 & 0.02318 & $0.008\pm0.010$ & $0.008\pm0.007$ & $-0.001\pm0.012$ & $0.06$ & $0.06$--$1.64$ & \ldots  & 169 & $-0.035$\,($0.65$) & $-0.021$\,($0.79$) & $-0.012$\,($0.81$) & $-0.26\pm0.55$ & $0.47$ & 0.089 \\
 & $\log$ sSFR$_{H\alpha}$ & 163 & -10.38 & $0.030\pm0.009$ & $-0.006\pm0.009$ & $-0.036\pm0.012$ & $2.91$ & $1.04$--$2.91$ & \ldots  & 163 & $-0.056$\,($0.48$) & $-0.099$\,($0.21$) & $-0.070$\,($0.18$) & $-0.0049\pm0.0066$ & $0.73$ & 0.089 \\
 & $\log$ sSFR$_{UV}$ & 169 & -9.713 & $0.030\pm0.009$ & $-0.004\pm0.009$ & $-0.035\pm0.012$ & $2.83$ & $2.09$--$4.32$ & $1.25$  & 119 & $-0.123$\,($0.18$) & $-0.164$\,($0.074$) & $-0.112$\,($0.071$) & $-0.0119\pm0.0094$ & $1.27$ & 0.089 \\
 & $\log t_L$ & 169 & 8.807 & $-0.005\pm0.008$ & $0.030\pm0.008$ & $0.035\pm0.012$ & $2.99$ & $1.73$--$4.62$ & \ldots  & 169 & $+0.251$\,($1{\times}10^{-3}$) & $+0.285$\,($2{\times}10^{-4}$) & $+0.193$\,($2{\times}10^{-4}$) & $0.0314\pm0.0088$ & $3.56$ & 0.086 \\
 & $\log t_M$ & 169 & 9.227 & $-0.008\pm0.008$ & $0.031\pm0.008$ & $0.038\pm0.012$ & $3.23$ & $2.22$--$4.95$ & \ldots  & 169 & $+0.255$\,($8{\times}10^{-4}$) & $+0.256$\,($8{\times}10^{-4}$) & $+0.167$\,($1{\times}10^{-3}$) & $0.0293\pm0.0088$ & $3.34$ & 0.085 \\
\hline
HR$_{SALT}$ & 12+$\log$ (O/H) & 163 & 8.684 & $0.008\pm0.016$ & $-0.015\pm0.018$ & $-0.023\pm0.024$ & $0.96$ & $0.15$--$1.62$ & \ldots  & 163 & $-0.089$\,($0.26$) & $-0.106$\,($0.18$) & $-0.074$\,($0.16$) & $-0.080\pm0.073$ & $1.09$ & 0.182 \\
 & F275W-$r$ & 166 & 2.151 & $0.008\pm0.014$ & $-0.010\pm0.018$ & $-0.018\pm0.023$ & $0.82$ & $0.14$--$1.19$ & $1.20$  & 117 & $-0.185$\,($0.045$) & $-0.179$\,($0.053$) & $-0.134$\,($0.032$) & $-0.022\pm0.012$ & $1.81$ & 0.184 \\
 & $\log \Sigma$SFR$_{H\alpha}$ & 163 & -3.145 & $-0.003\pm0.018$ & $0.004\pm0.017$ & $0.007\pm0.025$ & $0.29$ & $0.28$--$0.77$ & \ldots  & 163 & $-0.014$\,($0.86$) & $-0.013$\,($0.87$) & $-0.010$\,($0.85$) & $-0.002\pm0.015$ & $0.16$ & 0.183 \\
 & $\log \Sigma$SFR$_{UV}$ & 169 & -2.49 & $-0.011\pm0.014$ & $0.010\pm0.018$ & $0.021\pm0.023$ & $0.90$ & $0.04$--$1.49$ & $1.02$  & 119 & $+0.046$\,($0.62$) & $+0.006$\,($0.95$) & $+0.003$\,($0.96$) & $0.016\pm0.030$ & $0.55$ & 0.193 \\
 & $\log$ EW$_{H_\alpha}$ & 162 & 0.9167 & $-0.025\pm0.020$ & $0.017\pm0.014$ & $0.042\pm0.024$ & $1.73$ & $0.52$--$2.60$ & \ldots  & 162 & $+0.039$\,($0.63$) & $+0.077$\,($0.33$) & $+0.052$\,($0.33$) & $0.009\pm0.019$ & $0.48$ & 0.183 \\
 & $\log M$ & 169 & 7.907 & $0.009\pm0.014$ & $-0.035\pm0.018$ & $-0.044\pm0.023$ & $1.91$ & $0.29$--$1.97$ & \ldots  & 169 & $-0.085$\,($0.27$) & $-0.125$\,($0.11$) & $-0.092$\,($0.077$) & $-0.016\pm0.018$ & $0.91$ & 0.180 \\
 & $Z_L$ & 169 & 0.02498 & $0.017\pm0.015$ & $-0.019\pm0.018$ & $-0.036\pm0.023$ & $1.55$ & $1.06$--$2.36$ & \ldots  & 169 & $-0.049$\,($0.53$) & $-0.096$\,($0.22$) & $-0.067$\,($0.2$) & $-0.64\pm0.95$ & $0.68$ & 0.180 \\
 & $Z_M$ & 169 & 0.02318 & $0.029\pm0.017$ & $-0.021\pm0.015$ & $-0.050\pm0.022$ & $2.23$ & $0.00$--$2.23$ & \ldots  & 169 & $-0.072$\,($0.35$) & $-0.087$\,($0.26$) & $-0.062$\,($0.23$) & $-1.0\pm1.0$ & $0.97$ & 0.180 \\
 & $\log$ sSFR$_{H\alpha}$ & 163 & -10.38 & $-0.025\pm0.020$ & $0.025\pm0.014$ & $0.050\pm0.024$ & $2.06$ & $0.89$--$2.87$ & \ldots  & 163 & $+0.060$\,($0.44$) & $+0.112$\,($0.16$) & $+0.076$\,($0.15$) & $0.011\pm0.014$ & $0.78$ & 0.183 \\
 & $\log$ sSFR$_{UV}$ & 169 & -9.713 & $-0.035\pm0.018$ & $0.010\pm0.012$ & $0.045\pm0.022$ & $2.09$ & $1.45$--$2.12$ & $1.23$  & 119 & $+0.174$\,($0.058$) & $+0.226$\,($0.013$) & $+0.166$\,($8{\times}10^{-3}$) & $0.037\pm0.022$ & $1.72$ & 0.190 \\
 & $\log t_L$ & 169 & 8.807 & $0.009\pm0.013$ & $-0.026\pm0.018$ & $-0.035\pm0.022$ & $1.59$ & $0.56$--$2.57$ & \ldots  & 169 & $-0.112$\,($0.15$) & $-0.133$\,($0.085$) & $-0.093$\,($0.072$) & $-0.028\pm0.026$ & $1.10$ & 0.179 \\
 & $\log t_M$ & 169 & 9.227 & $0.019\pm0.014$ & $-0.036\pm0.017$ & $-0.055\pm0.022$ & $2.49$ & $0.87$--$3.28$ & \ldots  & 169 & $-0.160$\,($0.037$) & $-0.174$\,($0.024$) & $-0.122$\,($0.019$) & $-0.043\pm0.027$ & $1.56$ & 0.177 \\
\hline
\end{tabular}%
}
\end{sidewaystable*}

